Can one hear the shape of a neural network?: Snooping the GPU via Magnetic Side Channel

Neural network applications have become popular in both enterprise and personal settings. Network solutions are tuned meticulously for each task, and designs that can robustly resolve queries end up in high demand. As the commercial value of accurate and performant machine learning models increases, so too does the demand to protect neural architectures as confidential investments. We explore the vulnerability of neural networks deployed as black boxes across accelerated hardware through electromagnetic side channels. We examine the magnetic flux emanating from a graphics processing unit's power cable, as acquired by a cheap $3 induction sensor, and find that this signal betrays the detailed topology and hyperparameters of a black-box neural network model. The attack acquires the magnetic signal for one query with unknown input values, but known input dimensions. The network reconstruction is possible due to the modular layer sequence in which deep neural networks are evaluated. We find that each layer component's evaluation produces an identifiable magnetic signal signature, from which layer topology, width, function type, and sequence order can be inferred using a suitably trained classifier and a joint consistency optimization based on integer programming. We study the extent to which network specifications can be recovered, and consider metrics for comparing network similarity. We demonstrate the potential accuracy of this side channel attack in recovering the details for a broad range of network architectures, including random designs. We consider applications that may exploit this novel side channel exposure, such as adversarial transfer attacks. In response, we discuss countermeasures to protect against our method and other similar snooping techniques.

==> Makefile <==
# name of latex document
MAINDOC := NeuralSnoop_iclr2021

# latex source file
TEXSRC := NeuralSnoop_iclr2021.tex $(wildcard *.tex)
BIBSRC := $(wildcard *.bib)

ifneq ($(strip $(BIBSRC)),)
BBLSRC := $(MAINDOC).bbl
endif

# latex program
TEX      := latex
PDFLATEX := pdflatex
BIB      := bibtex

# flags
TEX_FLAGS :=
PDF_FLAGS :=
BIB_FLAGS :=

#=====================================================#
# Display Codes (this is so we can track passes)
#=====================================================#
MOVE_TO_COL	= @echo  "\\033[60G"
SETCOLOR_RED 	= @echo  "\\033[0;31m"
SETCOLOR_GREEN 	= @echo  "\\033[0;32m"
SETCOLOR_BLUE	= @echo  "\\033[0;34m"
SETCOLOR_BACK	= @echo  "\\033[0m"

all: $(MAINDOC).pdf

pdf: $(MAINDOC).pdf

dvi: $(MAINDOC).dvi

full: $(BBLSRC) $(TEXSRC)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)
	$(SETCOLOR_GREEN)
	@echo "=========================FINAL PASS=============================="
	$(SETCOLOR_BACK)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)


%.dvi : %.aux
	$(SETCOLOR_BLUE)
	@echo "=========================AUX -> DVI PASS=============================="
	$(SETCOLOR_BACK)
	@$(TEX) $(TEX_FLAGS) $(*F)
	
$(MAINDOC).bbl : $(BIBSRC) $(TEXSRC) 
ifneq ($(strip $(BIBSRC)),)
	$(SETCOLOR_GREEN)
	@echo "=========================LaTeX PASS=============================="
	$(SETCOLOR_BACK)
	$(PDFLATEX) $(TEX_FLAGS) $(MAINDOC)
	$(SETCOLOR_GREEN)
	@echo "=========================BibTex PASS=============================="
	$(SETCOLOR_BACK)
	@$(BIB) $(BIB_FLAGS) $(MAINDOC)
endif

$(MAINDOC).pdf : $(TEXSRC)
	$(SETCOLOR_GREEN)
	@echo "=========================SINGLE PASS=============================="
	$(SETCOLOR_BACK)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)

.PHONY: all clean

clean:
	-$(RM) *.aux *.pdf *.bbl *.blg *.log

